RankCLIP: Ranking-Consistent Language-Image Pretraining

Self-supervised contrastive learning models, such as CLIP, have set new benchmarks for vision-language models in many downstream tasks. However, their dependency on rigid one-to-one mappings overlooks the complex and often multifaceted relationships between and within texts and images. To this end, we introduce RankCLIP, a novel pre-training method that extends beyond the rigid one-to-one matching framework of CLIP and its variants. By extending the traditional pair-wise loss to list-wise, and leveraging both in-modal and cross-modal ranking consistency, RankCLIP improves the alignment process, enabling it to capture the nuanced many-to-many relationships between and within each modality. Through comprehensive experiments, we demonstrate the effectiveness of RankCLIP in various downstream tasks, notably achieving significant gains in zero-shot classifications over state-of-the-art methods, underscoring the importance of this enhanced learning process.

==> content/abstract.tex <==
\begin{abstract}
Self-supervised contrastive learning models, such as CLIP, have set new benchmarks for vision-language models in many downstream tasks.
%
However, their dependency on rigid one-to-one mappings overlooks the complex and often multifaceted relationships between and within texts and images. 
%
To this end, we introduce \textbf{\algname}, a novel pretraining method that extends beyond the rigid one-to-one matching framework of CLIP and its variants. 
%
By extending the traditional pair-wise contrastive loss to list-wise ranking consistency loss, and leveraging both in-modal and cross-modal ranking consistency, \algname improves the alignment process, enabling it to capture the nuanced many-to-many relationships between and within each modality.
%
Through comprehensive experiments, we demonstrate the effectiveness of \algname in various downstream tasks, achieving significant gains over state-of-the-art methods, underscoring the importance of this enhanced learning process.
%
\end{abstract}
